Elemental Abundances of Solar Sibling Candidates

Dynamical information along with survey data on metallicity and in some cases age have been used recently by some authors to search for candidates of stars that were born in the cluster where the Sun formed. We have acquired high resolution, high signal-to-noise ratio spectra for 30 of these objects to determine, using detailed elemental abundance analysis, if they could be true solar siblings. Only two of the candidates are found to have solar chemical composition. Updated modeling of the stars' past orbits in a realistic Galactic potential reveals that one of them, HD162826, satisfies both chemical and dynamical conditions for being a sibling of the Sun. Measurements of rare-element abundances for this star further confirm its solar composition, with the only possible exception of Sm. Analysis of long-term high-precision radial velocity data rules out the presence of hot Jupiters and confirms that this star is not in a binary system. We find that chemical tagging does not necessarily benefit from studying as many elements as possible, but instead from identifying and carefully measuring the abundances of those elements which show large star-to-star scatter at a given metallicity. Future searches employing data products from ongoing massive astrometric and spectroscopic surveys can be optimized by acknowledging this fact.

==> t2_full.tex <==
4779.44 & 26.0 & 3.42 & -2.16 \\
4788.76 & 26.0 & 3.24 & -1.73 \\
4799.41 & 26.0 & 3.64 & -2.13 \\
4808.15 & 26.0 & 3.25 & -2.69 \\
4961.91 & 26.0 & 3.63 & -2.19 \\
5044.211 & 26.0 & 2.851 & -2.058 \\
5054.64 & 26.0 & 3.64 & -1.98 \\
5187.91 & 26.0 & 4.14 & -1.26 \\
5197.94 & 26.0 & 4.3 & -1.54 \\
5198.71 & 26.0 & 2.22 & -2.14 \\
5242.49 & 26.0 & 3.63 & -0.99 \\
5243.77 & 26.0 & 4.26 & -0.99 \\
5288.52 & 26.0 & 3.69 & -1.51 \\
5295.31 & 26.0 & 4.42 & -1.59 \\
5321.1 & 26.0 & 4.43 & -1.26 \\
5322.04 & 26.0 & 2.28 & -2.89 \\
5373.71 & 26.0 & 4.47 & -0.74 \\
5379.57 & 26.0 & 3.69 & -1.51 \\
5386.33 & 26.0 & 4.15 & -1.67 \\
5441.34 & 26.0 & 4.31 & -1.63 \\
5522.45 & 26.0 & 4.21 & -1.45 \\
5543.94 & 26.0 & 4.22 & -1.04 \\
5546.51 & 26.0 & 4.37 & -1.21 \\
5554.89 & 26.0 & 4.55 & -0.36 \\
5560.21 & 26.0 & 4.43 & -1.09 \\
5618.63 & 26.0 & 4.21 & -1.27 \\
5638.26 & 26.0 & 4.22 & -0.77 \\
5651.469 & 26.0 & 4.473 & -1.75 \\
5679.023 & 26.0 & 4.652 & -0.75 \\
5696.09 & 26.0 & 4.548 & -1.72 \\
5705.464 & 26.0 & 4.301 & -1.355 \\
5731.76 & 26.0 & 4.26 & -1.2 \\
5775.08 & 26.0 & 4.22 & -1.3 \\
5778.453 & 26.0 & 2.588 & -3.44 \\
5793.914 & 26.0 & 4.22 & -1.619 \\
5806.73 & 26.0 & 4.61 & -0.95 \\
5809.218 & 26.0 & 3.883 & -1.71 \\
5852.22 & 26.0 & 4.55 & -1.23 \\
5855.076 & 26.0 & 4.608 & -1.478 \\
5856.09 & 26.0 & 4.29 & -1.46 \\
5859.59 & 26.0 & 4.55 & -0.58 \\
5905.67 & 26.0 & 4.65 & -0.69 \\
5909.97 & 26.0 & 3.21 & -2.6 \\
5916.25 & 26.0 & 2.45 & -2.99 \\
5927.79 & 26.0 & 4.65 & -0.99 \\
5929.68 & 26.0 & 4.55 & -1.31 \\
5930.18 & 26.0 & 4.65 & -0.17 \\
5934.65 & 26.0 & 3.93 & -1.07 \\
5956.694 & 26.0 & 0.859 & -4.552 \\
6003.01 & 26.0 & 3.88 & -1.06 \\
6027.05 & 26.0 & 4.076 & -1.09 \\
6056.0 & 26.0 & 4.73 & -0.4 \\
6065.482 & 26.0 & 2.609 & -1.53 \\
6079.01 & 26.0 & 4.65 & -1.02 \\
6082.71 & 26.0 & 2.22 & -3.57 \\
6085.26 & 26.0 & 2.76 & -3.05 \\
6093.644 & 26.0 & 4.607 & -1.3 \\
6096.665 & 26.0 & 3.984 & -1.81 \\
6127.91 & 26.0 & 4.14 & -1.4 \\
6151.618 & 26.0 & 2.176 & -3.282 \\
6157.72 & 26.0 & 4.07 & -1.2 \\
6165.36 & 26.0 & 4.143 & -1.46 \\
6173.335 & 26.0 & 2.223 & -2.88 \\
6187.99 & 26.0 & 3.94 & -1.62 \\
6200.313 & 26.0 & 2.609 & -2.416 \\
6213.43 & 26.0 & 2.223 & -2.52 \\
6219.28 & 26.0 & 2.2 & -2.43 \\
6229.23 & 26.0 & 2.85 & -2.83 \\
6232.64 & 26.0 & 3.65 & -1.22 \\
6240.646 & 26.0 & 2.223 & -3.287 \\
6246.32 & 26.0 & 3.6 & -0.87 \\
6252.555 & 26.0 & 2.404 & -1.687 \\
6265.134 & 26.0 & 2.176 & -2.547 \\
6270.225 & 26.0 & 2.858 & -2.54 \\
6322.69 & 26.0 & 2.59 & -2.43 \\
6335.33 & 26.0 & 2.2 & -2.26 \\
6336.82 & 26.0 & 3.69 & -0.93 \\
6358.68 & 26.0 & 0.86 & -4.24 \\
6380.74 & 26.0 & 4.19 & -1.32 \\
6393.6 & 26.0 & 2.43 & -1.6 \\
6430.846 & 26.0 & 2.176 & -2.006 \\
6481.87 & 26.0 & 2.28 & -2.98 \\
6498.939 & 26.0 & 0.958 & -4.695 \\
6574.229 & 26.0 & 0.99 & -5.01 \\
6593.871 & 26.0 & 2.433 & -2.394 \\
6597.56 & 26.0 & 4.8 & -0.97 \\
6609.11 & 26.0 & 2.559 & -2.682 \\
6703.567 & 26.0 & 2.759 & -3.023 \\
6705.102 & 26.0 & 4.607 & -0.98 \\
6713.745 & 26.0 & 4.795 & -1.4 \\
6726.667 & 26.0 & 4.607 & -1.03 \\
6739.522 & 26.0 & 1.557 & -4.794 \\
6750.152 & 26.0 & 2.424 & -2.621 \\
6752.71 & 26.0 & 4.64 & -1.22 \\
6810.263 & 26.0 & 4.607 & -0.986 \\
6828.59 & 26.0 & 4.64 & -0.82 \\
6837.006 & 26.0 & 4.593 & -1.687 \\
6843.66 & 26.0 & 4.55 & -0.83 \\
6858.15 & 26.0 & 4.61 & -0.94 \\
6945.205 & 26.0 & 2.424 & -2.454 \\
6999.88 & 26.0 & 4.1 & -1.46 \\
7090.38 & 26.0 & 4.23 & -1.11 \\
7132.99 & 26.0 & 4.08 & -1.65 \\
7401.685 & 26.0 & 4.186 & -1.5 \\
7418.67 & 26.0 & 4.14 & -1.38 \\
7583.79 & 26.0 & 3.02 & -1.88 \\
4491.4 & 26.1 & 2.856 & -2.66 \\
4508.29 & 26.1 & 2.856 & -2.52 \\
4576.333 & 26.1 & 2.844 & -2.95 \\
4620.513 & 26.1 & 2.828 & -3.21 \\
4993.34 & 26.1 & 2.81 & -3.73 \\
5132.66 & 26.1 & 2.81 & -4.17 \\
5197.577 & 26.1 & 3.231 & -2.22 \\
5234.624 & 26.1 & 3.221 & -2.18 \\
5264.804 & 26.1 & 3.23 & -3.13 \\
5325.55 & 26.1 & 3.22 & -3.25 \\
5414.072 & 26.1 & 3.221 & -3.58 \\
5425.257 & 26.1 & 3.2 & -3.22 \\
5534.84 & 26.1 & 3.24 & -2.88 \\
6084.09 & 26.1 & 3.2 & -3.83 \\
6149.24 & 26.1 & 3.89 & -2.75 \\
6238.38 & 26.1 & 3.89 & -2.63 \\
6247.55 & 26.1 & 3.89 & -2.38 \\
6369.462 & 26.1 & 2.891 & -4.11 \\
6432.676 & 26.1 & 2.891 & -3.57 \\
6516.077 & 26.1 & 2.891 & -3.31 \\
7515.831 & 26.1 & 3.903 & -3.39 \\


==> t4_full.tex <==
7771.9438 & 8.0 & 9.146 & 0.352 \\
7774.1611 & 8.0 & 9.146 & 0.223 \\
7775.3901 & 8.0 & 9.146 & 0.002 \\
5688.21 & 11.0 & 2.1 & -0.48 \\
6154.2251 & 11.0 & 2.102 & -1.547 \\
6160.7471 & 11.0 & 2.104 & -1.246 \\
5557.07 & 13.0 & 3.14 & -2.21 \\
6696.0181 & 13.0 & 3.143 & -1.481 \\
6698.667 & 13.0 & 3.143 & -1.782 \\
7835.309 & 13.0 & 4.022 & -0.689 \\
5517.54 & 14.0 & 5.08 & -2.496 \\
5645.6128 & 14.0 & 4.93 & -2.043 \\
5665.554 & 14.0 & 4.92 & -1.94 \\
5690.4248 & 14.0 & 4.93 & -1.773 \\
5701.105 & 14.0 & 4.93 & -1.953 \\
5772.145 & 14.0 & 5.082 & -1.653 \\
5793.0732 & 14.0 & 4.93 & -1.963 \\
5948.54 & 14.0 & 5.08 & -1.208 \\
6125.03 & 14.0 & 5.61 & -1.51 \\
6142.49 & 14.0 & 5.62 & -1.54 \\
6145.02 & 14.0 & 5.61 & -1.48 \\
6237.33 & 14.0 & 5.61 & -1.116 \\
6243.82 & 14.0 & 5.62 & -1.31 \\
6244.48 & 14.0 & 5.61 & -1.36 \\
6721.84 & 14.0 & 5.863 & -1.06 \\
6741.64 & 14.0 & 5.984 & -1.653 \\
7405.77 & 14.0 & 5.614 & -0.72 \\
7423.52 & 14.0 & 5.62 & -0.65 \\
7680.27 & 14.0 & 5.863 & -0.59 \\
7800.0 & 14.0 & 6.18 & -0.71 \\
4512.2681 & 20.0 & 2.526 & -1.901 \\
5349.47 & 20.0 & 2.71 & -0.581 \\
5512.98 & 20.0 & 2.93 & -0.559 \\
5581.97 & 20.0 & 2.52 & -0.63 \\
5590.12 & 20.0 & 2.52 & -0.65 \\
5867.562 & 20.0 & 2.933 & -1.57 \\
6156.02 & 20.0 & 2.52 & -2.497 \\
6161.2969 & 20.0 & 2.523 & -1.266 \\
6166.439 & 20.0 & 2.521 & -1.142 \\
6169.042 & 20.0 & 2.523 & -0.797 \\
6169.55 & 20.0 & 2.52 & -0.58 \\
6455.5981 & 20.0 & 2.523 & -1.34 \\
6471.6621 & 20.0 & 2.526 & -0.686 \\
6499.6499 & 20.0 & 2.523 & -0.818 \\
6572.8 & 20.0 & 0.0 & -4.28 \\
5318.374 & 21.1 & 1.357 & -2.015 \\
5526.82 & 21.1 & 1.77 & 0.14 \\
5657.88 & 21.1 & 1.51 & -0.326 \\
6245.6411 & 21.1 & 1.507 & -1.036 \\
6604.5781 & 21.1 & 1.357 & -1.309 \\
4758.118 & 22.0 & 2.249 & 0.481 \\
4759.269 & 22.0 & 2.256 & 0.57 \\
4778.258 & 22.0 & 2.236 & -0.22 \\
5219.699 & 22.0 & 0.021 & -2.236 \\
5426.26 & 22.0 & 0.02 & -2.95 \\
5471.2 & 22.0 & 1.44 & -1.4 \\
5739.464 & 22.0 & 2.249 & -0.6 \\
5978.55 & 22.0 & 1.87 & -0.602 \\
6126.217 & 22.0 & 1.066 & -1.424 \\
6258.099 & 22.0 & 1.443 & -0.299 \\
6261.101 & 22.0 & 1.429 & -0.479 \\
5336.778 & 22.1 & 1.582 & -1.63 \\
5418.7675 & 22.1 & 1.582 & -2.11 \\
5670.832 & 23.0 & 1.08 & -3.402 \\
-5670.832 & 23.0 & 1.08 & -2.101 \\
-5670.832 & 23.0 & 1.08 & -1.093 \\
-5670.844 & 23.0 & 1.08 & -3.004 \\
-5670.844 & 23.0 & 1.08 & -1.891 \\
-5670.844 & 23.0 & 1.08 & -1.198 \\
-5670.854 & 23.0 & 1.08 & -2.8 \\
-5670.854 & 23.0 & 1.08 & -1.817 \\
-5670.854 & 23.0 & 1.08 & -1.314 \\
-5670.863 & 23.0 & 1.08 & -2.703 \\
-5670.863 & 23.0 & 1.08 & -1.811 \\
-5670.863 & 23.0 & 1.08 & -1.443 \\
-5670.87 & 23.0 & 1.08 & -2.703 \\
-5670.87 & 23.0 & 1.08 & -1.858 \\
-5670.87 & 23.0 & 1.08 & -1.589 \\
-5670.875 & 23.0 & 1.08 & -2.858 \\
-5670.875 & 23.0 & 1.08 & -1.963 \\
-5670.875 & 23.0 & 1.08 & -1.759 \\
-5670.878 & 23.0 & 1.08 & -2.159 \\
-5670.878 & 23.0 & 1.08 & -1.963 \\
-5670.88 & 23.0 & 1.08 & -2.226 \\
5703.5552 & 23.0 & 1.0509 & -0.779 \\
-5703.5688 & 23.0 & 1.0509 & -0.995 \\
-5703.5688 & 23.0 & 1.0509 & -1.405 \\
-5703.5796 & 23.0 & 1.0509 & -1.244 \\
-5703.5796 & 23.0 & 1.0509 & -1.278 \\
-5703.5811 & 23.0 & 1.0509 & -2.27 \\
-5703.5889 & 23.0 & 1.0509 & -1.717 \\
-5703.5889 & 23.0 & 1.0509 & -1.252 \\
-5703.5898 & 23.0 & 1.0509 & -1.842 \\
-5703.5962 & 23.0 & 1.0509 & -1.592 \\
-5703.5962 & 23.0 & 1.0509 & -1.416 \\
-5703.6011 & 23.0 & 1.0509 & -1.416 \\
5727.027 & 23.0 & 1.081 & -2.993 \\
-5727.027 & 23.0 & 1.081 & -1.692 \\
-5727.027 & 23.0 & 1.081 & -0.684 \\
-5727.039 & 23.0 & 1.081 & -2.595 \\
-5727.039 & 23.0 & 1.081 & -1.481 \\
-5727.039 & 23.0 & 1.081 & -0.789 \\
-5727.049 & 23.0 & 1.081 & -2.391 \\
-5727.049 & 23.0 & 1.081 & -1.408 \\
-5727.049 & 23.0 & 1.081 & -0.905 \\
-5727.058 & 23.0 & 1.081 & -2.294 \\
-5727.058 & 23.0 & 1.081 & -1.402 \\
-5727.058 & 23.0 & 1.081 & -1.034 \\
-5727.065 & 23.0 & 1.081 & -2.294 \\
-5727.065 & 23.0 & 1.081 & -1.449 \\
-5727.065 & 23.0 & 1.081 & -1.18 \\
-5727.07 & 23.0 & 1.081 & -2.449 \\
-5727.07 & 23.0 & 1.081 & -1.554 \\
-5727.07 & 23.0 & 1.081 & -1.35 \\
-5727.074 & 23.0 & 1.081 & -1.75 \\
-5727.074 & 23.0 & 1.081 & -1.554 \\
-5727.076 & 23.0 & 1.081 & -1.817 \\
5727.6191 & 23.0 & 1.0509 & -1.892 \\
-5727.6191 & 23.0 & 1.0509 & -1.481 \\
-5727.6533 & 23.0 & 1.0509 & -2.097 \\
-5727.6533 & 23.0 & 1.0509 & -1.778 \\
-5727.6538 & 23.0 & 1.0509 & -1.892 \\
-5727.6812 & 23.0 & 1.0509 & -1.903 \\
-5727.6812 & 23.0 & 1.0509 & -1.778 \\
-5727.7007 & 23.0 & 1.0509 & -2.079 \\
-5727.7021 & 23.0 & 1.0509 & -1.903 \\
5737.0269 & 23.0 & 1.0636 & -1.382 \\
-5737.0366 & 23.0 & 1.0636 & -2.081 \\
-5737.041 & 23.0 & 1.0636 & -2.081 \\
-5737.0508 & 23.0 & 1.0636 & -1.674 \\
-5737.0586 & 23.0 & 1.0636 & -1.9 \\
-5737.063 & 23.0 & 1.0636 & -1.9 \\
-5737.0708 & 23.0 & 1.0636 & -2.08 \\
-5737.0771 & 23.0 & 1.0636 & -1.869 \\
-5737.0801 & 23.0 & 1.0636 & -1.869 \\
-5737.0859 & 23.0 & 1.0636 & -2.797 \\
-5737.0908 & 23.0 & 1.0636 & -1.933 \\
-5737.0928 & 23.0 & 1.0636 & -1.933 \\
-5737.0977 & 23.0 & 1.0636 & -4.04 \\
-5737.1006 & 23.0 & 1.0636 & -2.132 \\
-5737.1035 & 23.0 & 1.0636 & -2.132 \\
-5737.1055 & 23.0 & 1.0636 & -2.387 \\
6039.727 & 23.0 & 1.063 & -1.854 \\
-6039.729 & 23.0 & 1.063 & -1.854 \\
-6039.73 & 23.0 & 1.063 & -2.03 \\
-6039.733 & 23.0 & 1.063 & -1.69 \\
-6039.733 & 23.0 & 1.063 & -2.155 \\
-6039.734 & 23.0 & 1.063 & -2.28 \\
-6039.738 & 23.0 & 1.063 & -1.682 \\
-6039.738 & 23.0 & 1.063 & -1.716 \\
-6039.739 & 23.0 & 1.063 & -2.708 \\
-6039.744 & 23.0 & 1.063 & -1.843 \\
-6039.744 & 23.0 & 1.063 & -1.433 \\
-6039.751 & 23.0 & 1.063 & -1.217 \\
6090.199 & 23.0 & 1.08 & -0.692 \\
-6090.207 & 23.0 & 1.08 & -0.833 \\
-6090.213 & 23.0 & 1.08 & -0.997 \\
-6090.213 & 23.0 & 1.08 & -1.532 \\
-6090.218 & 23.0 & 1.08 & -1.195 \\
-6090.218 & 23.0 & 1.08 & -1.336 \\
-6090.223 & 23.0 & 1.08 & -1.45 \\
-6090.223 & 23.0 & 1.08 & -1.282 \\
-6090.225 & 23.0 & 1.08 & -2.646 \\
-6090.226 & 23.0 & 1.08 & -1.304 \\
-6090.227 & 23.0 & 1.08 & -1.838 \\
-6090.228 & 23.0 & 1.08 & -2.236 \\
-6090.229 & 23.0 & 1.08 & -1.394 \\
-6090.231 & 23.0 & 1.08 & -1.583 \\
-6090.231 & 23.0 & 1.08 & -2.014 \\
-6090.232 & 23.0 & 1.08 & -1.889 \\
-6090.233 & 23.0 & 1.08 & -1.868 \\
-6090.233 & 23.0 & 1.08 & -1.838 \\
6199.155 & 23.0 & 0.286 & -1.958 \\
-6199.173 & 23.0 & 0.286 & -2.063 \\
-6199.188 & 23.0 & 0.286 & -2.179 \\
-6199.203 & 23.0 & 0.286 & -2.308 \\
-6199.207 & 23.0 & 0.286 & -2.966 \\
-6199.215 & 23.0 & 0.286 & -2.454 \\
-6199.218 & 23.0 & 0.286 & -2.755 \\
-6199.226 & 23.0 & 0.286 & -2.624 \\
-6199.227 & 23.0 & 0.286 & -2.682 \\
-6199.235 & 23.0 & 0.286 & -2.676 \\
-6199.236 & 23.0 & 0.286 & -2.828 \\
-6199.241 & 23.0 & 0.286 & -2.723 \\
-6199.244 & 23.0 & 0.286 & -3.091 \\
-6199.246 & 23.0 & 0.286 & -2.828 \\
-6199.249 & 23.0 & 0.286 & -3.024 \\
-6199.252 & 23.0 & 0.286 & -4.267 \\
-6199.256 & 23.0 & 0.286 & -3.869 \\
-6199.259 & 23.0 & 0.286 & -3.723 \\
-6199.259 & 23.0 & 0.286 & -3.665 \\
-6199.26 & 23.0 & 0.286 & -3.568 \\
-6199.261 & 23.0 & 0.286 & -3.568 \\
6224.4609 & 23.0 & 0.2866 & -3.519 \\
-6224.4707 & 23.0 & 0.2866 & -3.315 \\
-6224.48 & 23.0 & 0.2866 & -3.25 \\
-6224.4893 & 23.0 & 0.2866 & -3.257 \\
-6224.4961 & 23.0 & 0.2866 & -2.616 \\
-6224.4961 & 23.0 & 0.2866 & -3.323 \\
-6224.501 & 23.0 & 0.2866 & -2.803 \\
-6224.5029 & 23.0 & 0.2866 & -3.461 \\
-6224.5049 & 23.0 & 0.2866 & -3.022 \\
-6224.5078 & 23.0 & 0.2866 & -3.285 \\
-6224.5098 & 23.0 & 0.2866 & -3.741 \\
-6224.5112 & 23.0 & 0.2866 & -3.616 \\
-6224.5127 & 23.0 & 0.2866 & -4.063 \\
-6224.5146 & 23.0 & 0.2866 & -4.762 \\
-6224.5205 & 23.0 & 0.2866 & -3.741 \\
-6224.5239 & 23.0 & 0.2866 & -3.461 \\
-6224.5283 & 23.0 & 0.2866 & -3.323 \\
-6224.5312 & 23.0 & 0.2866 & -3.257 \\
-6224.5332 & 23.0 & 0.2866 & -3.25 \\
-6224.5342 & 23.0 & 0.2866 & -3.315 \\
-6224.5352 & 23.0 & 0.2866 & -3.519 \\
6274.607 & 23.0 & 0.267 & -2.932 \\
-6274.629 & 23.0 & 0.267 & -2.455 \\
-6274.641 & 23.0 & 0.267 & -2.476 \\
-6274.655 & 23.0 & 0.267 & -2.134 \\
-6274.657 & 23.0 & 0.267 & -2.455 \\
-6274.678 & 23.0 & 0.267 & -2.601 \\
6285.098 & 23.0 & 0.275 & -3.568 \\
-6285.117 & 23.0 & 0.275 & -3.14 \\
-6285.122 & 23.0 & 0.275 & -2.703 \\
-6285.134 & 23.0 & 0.275 & -2.89 \\
-6285.137 & 23.0 & 0.275 & -2.542 \\
-6285.148 & 23.0 & 0.275 & -2.714 \\
-6285.149 & 23.0 & 0.275 & -2.55 \\
-6285.152 & 23.0 & 0.275 & -2.077 \\
-6285.157 & 23.0 & 0.275 & -2.714 \\
-6285.162 & 23.0 & 0.275 & -2.293 \\
-6285.168 & 23.0 & 0.275 & -2.576 \\
-6285.172 & 23.0 & 0.275 & -3.015 \\
4936.3355 & 24.0 & 3.113 & -0.237 \\
5214.14 & 24.0 & 3.37 & -0.784 \\
5238.96 & 24.0 & 2.71 & -1.43 \\
5296.691 & 24.0 & 0.983 & -1.41 \\
5783.073 & 24.0 & 3.232 & -0.48 \\
5783.87 & 24.0 & 3.322 & -0.29 \\
5787.93 & 24.0 & 3.322 & -0.08 \\
6330.1 & 24.0 & 0.941 & -2.9 \\
6882.4772 & 24.0 & 3.438 & -0.375 \\
6882.997 & 24.0 & 3.438 & -0.42 \\
4588.1997 & 24.1 & 4.071 & -0.594 \\
5237.328 & 24.1 & 4.073 & -1.087 \\
5305.87 & 24.1 & 3.827 & -1.97 \\
5308.42 & 24.1 & 4.07 & -1.79 \\
4709.693 & 25.0 & 2.8884 & -0.949 \\
-4709.698 & 25.0 & 2.8884 & -1.94 \\
-4709.701 & 25.0 & 2.8884 & -1.94 \\
-4709.706 & 25.0 & 2.8884 & -1.119 \\
-4709.711 & 25.0 & 2.8884 & -1.758 \\
-4709.713 & 25.0 & 2.8884 & -1.758 \\
-4709.717 & 25.0 & 2.8884 & -1.304 \\
-4709.721 & 25.0 & 2.8884 & -1.727 \\
-4709.723 & 25.0 & 2.8884 & -1.727 \\
-4709.726 & 25.0 & 2.8884 & -1.496 \\
-4709.729 & 25.0 & 2.8884 & -1.792 \\
-4709.73 & 25.0 & 2.8884 & -1.792 \\
-4709.733 & 25.0 & 2.8884 & -1.671 \\
-4709.735 & 25.0 & 2.8884 & -1.99 \\
-4709.736 & 25.0 & 2.8884 & -1.99 \\
-4709.737 & 25.0 & 2.8884 & -1.735 \\
5394.6191 & 25.0 & 0.0 & -4.067 \\
-5394.6509 & 25.0 & 0.0 & -4.985 \\
-5394.6538 & 25.0 & 0.0 & -4.207 \\
-5394.6772 & 25.0 & 0.0 & -6.202 \\
-5394.6807 & 25.0 & 0.0 & -4.809 \\
-5394.6831 & 25.0 & 0.0 & -4.365 \\
-5394.7021 & 25.0 & 0.0 & -5.85 \\
-5394.7051 & 25.0 & 0.0 & -4.783 \\
-5394.707 & 25.0 & 0.0 & -4.549 \\
-5394.7212 & 25.0 & 0.0 & -5.725 \\
-5394.7227 & 25.0 & 0.0 & -4.85 \\
-5394.7246 & 25.0 & 0.0 & -4.771 \\
-5394.7339 & 25.0 & 0.0 & -5.804 \\
-5394.7358 & 25.0 & 0.0 & -5.056 \\
-5394.7358 & 25.0 & 0.0 & -5.026 \\
5399.45 & 25.0 & 3.85 & -1.162 \\
-5399.455 & 25.0 & 3.85 & -1.03 \\
-5399.465 & 25.0 & 3.85 & -1.53 \\
-5399.465 & 25.0 & 3.85 & -1.132 \\
-5399.478 & 25.0 & 3.85 & -2.74 \\
-5399.494 & 25.0 & 3.85 & -1.162 \\
-5399.497 & 25.0 & 3.85 & -1.204 \\
-5399.521 & 25.0 & 3.85 & -1.03 \\
-5399.522 & 25.0 & 3.85 & -0.655 \\
-5399.555 & 25.0 & 3.85 & -1.132 \\
5413.5933 & 25.0 & 3.859 & -1.81 \\
-5413.6279 & 25.0 & 3.859 & -1.379 \\
-5413.6377 & 25.0 & 3.859 & -1.266 \\
-5413.6577 & 25.0 & 3.859 & -1.266 \\
-5413.6968 & 25.0 & 3.859 & -0.902 \\
-5413.7017 & 25.0 & 3.859 & -1.363 \\
6013.52 & 25.0 & 3.073 & -0.765 \\
-6013.545 & 25.0 & 3.073 & -0.977 \\
-6013.567 & 25.0 & 3.073 & -1.25 \\
-6013.573 & 25.0 & 3.073 & -1.454 \\
-6013.584 & 25.0 & 3.073 & -1.66 \\
-6013.587 & 25.0 & 3.073 & -1.308 \\
-6013.598 & 25.0 & 3.073 & -1.329 \\
-6013.605 & 25.0 & 3.073 & -1.484 \\
-6013.615 & 25.0 & 3.073 & -2.408 \\
-6013.615 & 25.0 & 3.073 & -1.806 \\
-6013.619 & 25.0 & 3.073 & -2.028 \\
-6013.619 & 25.0 & 3.073 & -1.852 \\
6016.613 & 25.0 & 3.073 & -1.444 \\
-6016.64 & 25.0 & 3.073 & -0.666 \\
-6016.64 & 25.0 & 3.073 & -1.281 \\
-6016.661 & 25.0 & 3.073 & -1.276 \\
-6016.662 & 25.0 & 3.073 & -0.929 \\
-6016.678 & 25.0 & 3.073 & -1.378 \\
-6016.679 & 25.0 & 3.073 & -1.26 \\
-6016.689 & 25.0 & 3.073 & -1.444 \\
-6016.69 & 25.0 & 3.073 & -1.707 \\
-6016.691 & 25.0 & 3.073 & -1.64 \\
-6016.697 & 25.0 & 3.073 & -2.406 \\
-6016.701 & 25.0 & 3.073 & -1.281 \\
-6016.707 & 25.0 & 3.073 & -1.64 \\
-6016.708 & 25.0 & 3.073 & -1.276 \\
-6016.709 & 25.0 & 3.073 & -1.378 \\
6021.746 & 25.0 & 3.075 & -2.668 \\
-6021.772 & 25.0 & 3.075 & -1.451 \\
-6021.774 & 25.0 & 3.075 & -2.316 \\
-6021.795 & 25.0 & 3.075 & -1.275 \\
-6021.798 & 25.0 & 3.075 & -2.191 \\
-6021.804 & 25.0 & 3.075 & -0.533 \\
-6021.813 & 25.0 & 3.075 & -1.249 \\
-6021.817 & 25.0 & 3.075 & -2.271 \\
-6021.821 & 25.0 & 3.075 & -0.673 \\
-6021.827 & 25.0 & 3.075 & -1.316 \\
-6021.834 & 25.0 & 3.075 & -0.831 \\
-6021.837 & 25.0 & 3.075 & -1.492 \\
-6021.843 & 25.0 & 3.075 & -1.015 \\
-6021.846 & 25.0 & 3.075 & -1.522 \\
-6021.847 & 25.0 & 3.075 & -1.237 \\
5342.706 & 27.0 & 4.021 & -0.187 \\
-5342.693 & 27.0 & 4.021 & -0.743 \\
-5342.693 & 27.0 & 4.021 & -0.66 \\
-5342.693 & 27.0 & 4.021 & -0.574 \\
-5342.694 & 27.0 & 4.021 & -0.49 \\
-5342.696 & 27.0 & 4.021 & -0.408 \\
-5342.699 & 27.0 & 4.021 & -0.331 \\
-5342.701 & 27.0 & 4.021 & -1.468 \\
-5342.702 & 27.0 & 4.021 & -0.257 \\
-5342.704 & 27.0 & 4.021 & -1.25 \\
-5342.707 & 27.0 & 4.021 & -1.156 \\
-5342.712 & 27.0 & 4.021 & -1.124 \\
-5342.713 & 27.0 & 4.021 & -2.681 \\
-5342.716 & 27.0 & 4.021 & -1.144 \\
-5342.718 & 27.0 & 4.021 & -2.447 \\
-5342.722 & 27.0 & 4.021 & -1.231 \\
-5342.725 & 27.0 & 4.021 & -2.401 \\
-5342.728 & 27.0 & 4.021 & -1.454 \\
-5342.732 & 27.0 & 4.021 & -2.468 \\
-5342.739 & 27.0 & 4.021 & -2.651 \\
-5342.748 & 27.0 & 4.021 & -3.033 \\
5647.232 & 27.0 & 2.28 & -2.626 \\
-5647.207 & 27.0 & 2.28 & -2.127 \\
-5647.22 & 27.0 & 2.28 & -2.343 \\
-5647.239 & 27.0 & 2.28 & -2.753 \\
-5647.243 & 27.0 & 2.28 & -3.065 \\
-5647.246 & 27.0 & 2.28 & -2.592 \\
-5647.253 & 27.0 & 2.28 & -2.6 \\
-5647.259 & 27.0 & 2.28 & -2.764 \\
-5647.265 & 27.0 & 2.28 & -3.618 \\
-5647.267 & 27.0 & 2.28 & -3.19 \\
-5647.269 & 27.0 & 2.28 & -2.764 \\
-5647.269 & 27.0 & 2.28 & -2.94 \\
6093.1484 & 27.0 & 1.7403 & -3.468 \\
-6093.0952 & 27.0 & 1.7403 & -3.457 \\
-6093.1157 & 27.0 & 1.7403 & -3.046 \\
-6093.124 & 27.0 & 1.7403 & -3.343 \\
-6093.1392 & 27.0 & 1.7403 & -3.662 \\
-6093.1597 & 27.0 & 1.7403 & -3.457 \\
-6093.1738 & 27.0 & 1.7403 & -3.644 \\
-6093.1738 & 27.0 & 1.7403 & -3.343 \\
-6093.1846 & 27.0 & 1.7403 & -3.468 \\
6188.925 & 27.0 & 1.71 & -3.805 \\
-6188.937 & 27.0 & 1.71 & -3.106 \\
-6188.968 & 27.0 & 1.71 & -3.624 \\
-6188.979 & 27.0 & 1.71 & -3.398 \\
-6188.991 & 27.0 & 1.71 & -3.805 \\
-6189.003 & 27.0 & 1.71 & -3.593 \\
-6189.012 & 27.0 & 1.71 & -3.804 \\
-6189.024 & 27.0 & 1.71 & -3.624 \\
-6189.03 & 27.0 & 1.71 & -3.657 \\
-6189.038 & 27.0 & 1.71 & -4.521 \\
-6189.048 & 27.0 & 1.71 & -3.593 \\
-6189.052 & 27.0 & 1.71 & -3.856 \\
-6189.057 & 27.0 & 1.71 & -5.764 \\
-6189.065 & 27.0 & 1.71 & -3.657 \\
-6189.069 & 27.0 & 1.71 & -4.111 \\
-6189.075 & 27.0 & 1.71 & -3.856 \\
6454.946 & 27.0 & 3.632 & -1.4194 \\
-6454.934 & 27.0 & 3.632 & -2.0562 \\
-6454.944 & 27.0 & 3.632 & -1.9892 \\
-6454.933 & 27.0 & 3.632 & -1.7929 \\
-6454.965 & 27.0 & 3.632 & -2.6882 \\
-6454.954 & 27.0 & 3.632 & -1.7929 \\
-6454.937 & 27.0 & 3.632 & -1.5888 \\
-6454.985 & 27.0 & 3.632 & -2.5333 \\
-6454.968 & 27.0 & 3.632 & -1.6882 \\
-6455.01 & 27.0 & 3.632 & -2.5333 \\
-6454.987 & 27.0 & 3.632 & -1.6412 \\
-6454.959 & 27.0 & 3.632 & -1.2732 \\
-6455.04 & 27.0 & 3.632 & -2.6302 \\
-6455.012 & 27.0 & 3.632 & -1.6468 \\
-6454.978 & 27.0 & 3.632 & -1.1441 \\
-6455.074 & 27.0 & 3.632 & -2.8343 \\
-6455.041 & 27.0 & 3.632 & -1.7204 \\
-6455.002 & 27.0 & 3.632 & -1.0282 \\
-6455.114 & 27.0 & 3.632 & -3.2323 \\
-6455.075 & 27.0 & 3.632 & -1.9312 \\
-6455.03 & 27.0 & 3.632 & -0.9226 \\
6814.9688 & 27.0 & 1.9557 & -3.026 \\
-6814.8887 & 27.0 & 1.9557 & -2.839 \\
-6814.915 & 27.0 & 1.9557 & -2.725 \\
-6814.9238 & 27.0 & 1.9557 & -2.428 \\
-6814.936 & 27.0 & 1.9557 & -2.85 \\
-6814.9434 & 27.0 & 1.9557 & -3.044 \\
-6814.978 & 27.0 & 1.9557 & -2.839 \\
-6814.9873 & 27.0 & 1.9557 & -2.725 \\
-6814.9907 & 27.0 & 1.9557 & -2.85 \\
7417.3853 & 27.0 & 2.0421 & -3.263 \\
-7417.3076 & 27.0 & 2.0421 & -2.637 \\
-7417.3491 & 27.0 & 2.0421 & -2.853 \\
-7417.3838 & 27.0 & 2.0421 & -3.136 \\
-7417.4126 & 27.0 & 2.0421 & -3.102 \\
-7417.4141 & 27.0 & 2.0421 & -3.575 \\
-7417.4355 & 27.0 & 2.0421 & -3.11 \\
-7417.4487 & 27.0 & 2.0421 & -4.128 \\
-7417.4517 & 27.0 & 2.0421 & -3.274 \\
-7417.4639 & 27.0 & 2.0421 & -3.7 \\
-7417.4736 & 27.0 & 2.0421 & -3.45 \\
-7417.4766 & 27.0 & 2.0421 & -3.274 \\
4953.21 & 28.0 & 3.74 & -0.58 \\
5010.94 & 28.0 & 3.63 & -0.901 \\
5082.35 & 28.0 & 3.658 & -0.59 \\
5094.42 & 28.0 & 3.833 & -1.07 \\
5102.97 & 28.0 & 1.68 & -2.66 \\
5593.746 & 28.0 & 3.899 & -0.78 \\
5748.36 & 28.0 & 1.68 & -3.24 \\
5805.22 & 28.0 & 4.168 & -0.62 \\
5847.01 & 28.0 & 1.676 & -3.41 \\
5996.74 & 28.0 & 4.236 & -1.01 \\
6007.317 & 28.0 & 1.677 & -3.41 \\
6086.288 & 28.0 & 4.266 & -0.46 \\
6108.12 & 28.0 & 1.68 & -2.43 \\
6111.08 & 28.0 & 4.088 & -0.81 \\
6130.14 & 28.0 & 4.266 & -0.94 \\
6175.37 & 28.0 & 4.089 & -0.55 \\
6176.798 & 28.0 & 4.088 & -0.26 \\
6177.25 & 28.0 & 1.826 & -3.51 \\
6186.717 & 28.0 & 4.106 & -0.88 \\
6204.6048 & 28.0 & 4.088 & -1.1 \\
6223.9914 & 28.0 & 4.105 & -1.052 \\
-6223.971 & 28.0 & 4.105 & -1.466 \\
6327.6 & 28.0 & 1.68 & -3.06 \\
6378.258 & 28.0 & 4.154 & -0.972 \\
-6378.2328 & 28.0 & 4.154 & -1.386 \\
6482.81 & 28.0 & 1.93 & -2.76 \\
6598.611 & 28.0 & 4.236 & -0.91 \\
6635.13 & 28.0 & 4.42 & -0.72 \\
6643.64 & 28.0 & 1.676 & -2.03 \\
6767.78 & 28.0 & 1.83 & -2.1 \\
6772.32 & 28.0 & 3.658 & -0.97 \\
7788.93 & 28.0 & 1.95 & -1.75 \\
7826.77 & 28.0 & 3.7 & -1.84 \\
4883.685 & 39.1 & 1.0841 & -0.298 \\
-4883.685 & 39.1 & 1.0841 & -1.729 \\
-4883.685 & 39.1 & 1.0841 & -0.185 \\
5087.418 & 39.1 & 1.0841 & -0.534 \\
-5087.418 & 39.1 & 1.0841 & -2.078 \\
-5087.42 & 39.1 & 1.0841 & -2.078 \\
-5087.42 & 39.1 & 1.0841 & -0.435 \\
5200.411 & 39.1 & 0.9923 & -1.968 \\
-5200.413 & 39.1 & 0.9923 & -1.014 \\
-5200.413 & 39.1 & 0.9923 & -0.822 \\
-5200.414 & 39.1 & 0.9923 & -1.968 \\
5402.7729 & 39.1 & 1.839 & -1.984 \\
-5402.7739 & 39.1 & 1.839 & -0.838 \\
-5402.7754 & 39.1 & 1.839 & -0.683 \\
5853.696 & 56.1 & 0.604 & -2.915 \\
-5853.697 & 56.1 & 0.604 & -2.857 \\
-5853.697 & 56.1 & 0.604 & -3.148 \\
-5853.698 & 56.1 & 0.604 & -3.09 \\
-5853.699 & 56.1 & 0.604 & -3.295 \\
-5853.699 & 56.1 & 0.604 & -3.061 \\
-5853.7 & 56.1 & 0.604 & -2.76 \\
-5853.7 & 56.1 & 0.604 & -3.693 \\
-5853.7 & 56.1 & 0.604 & -2.546 \\
-5853.7 & 56.1 & 0.604 & -2.53 \\
-5853.7 & 56.1 & 0.604 & -3.459 \\
-5853.7 & 56.1 & 0.604 & -2.313 \\
-5853.7 & 56.1 & 0.604 & -1.054 \\
-5853.7 & 56.1 & 0.604 & -2.012 \\
-5853.7 & 56.1 & 0.604 & -2.994 \\
-5853.701 & 56.1 & 0.604 & -3.295 \\
-5853.702 & 56.1 & 0.604 & -3.061 \\
-5853.703 & 56.1 & 0.604 & -2.857 \\
-5853.703 & 56.1 & 0.604 & -3.09 \\
-5853.704 & 56.1 & 0.604 & -3.148 \\
-5853.704 & 56.1 & 0.604 & -2.915 \\
6141.695 & 56.1 & 0.704 & -3.641 \\
-6141.695 & 56.1 & 0.704 & -3.407 \\
-6141.697 & 56.1 & 0.704 & -2.495 \\
-6141.697 & 56.1 & 0.704 & -2.261 \\
-6141.698 & 56.1 & 0.704 & -3.465 \\
-6141.698 & 56.1 & 0.704 & -3.231 \\
-6141.699 & 56.1 & 0.704 & -1.686 \\
-6141.699 & 56.1 & 0.704 & -1.453 \\
-6141.699 & 56.1 & 0.704 & -2.398 \\
-6141.699 & 56.1 & 0.704 & -2.164 \\
-6141.7 & 56.1 & 0.704 & -1.7 \\
-6141.7 & 56.1 & 0.704 & -0.224 \\
-6141.7 & 56.1 & 0.704 & -1.182 \\
-6141.701 & 56.1 & 0.704 & -1.892 \\
-6141.701 & 56.1 & 0.704 & -1.659 \\
-6141.701 & 56.1 & 0.704 & -2.51 \\
-6141.701 & 56.1 & 0.704 & -2.277 \\
-6141.702 & 56.1 & 0.704 & -1.909 \\
-6141.702 & 56.1 & 0.704 & -2.465 \\
-6141.702 & 56.1 & 0.704 & -2.143 \\
-6141.703 & 56.1 & 0.704 & -2.231 \\
6496.9 & 56.1 & 0.604 & -2.0 \\
-6496.906 & 56.1 & 0.604 & -2.764 \\
-6496.907 & 56.1 & 0.604 & -2.367 \\
-6496.889 & 56.1 & 0.604 & -3.066 \\
-6496.91 & 56.1 & 0.604 & -2.367 \\
-6496.892 & 56.1 & 0.604 & -2.367 \\
-6496.896 & 56.1 & 0.604 & -1.919 \\
-6496.9 & 56.1 & 0.604 & -1.482 \\
-6496.906 & 56.1 & 0.604 & -2.531 \\
-6496.908 & 56.1 & 0.604 & -2.133 \\
-6496.888 & 56.1 & 0.604 & -2.832 \\
-6496.912 & 56.1 & 0.604 & -2.133 \\
-6496.891 & 56.1 & 0.604 & -2.133 \\
-6496.896 & 56.1 & 0.604 & -1.686 \\
-6496.9 & 56.1 & 0.604 & -0.524 \\

